MARGIN: Uncovering Deep Neural Networks using Graph Signal Analysis

Interpretability has emerged as a crucial aspect of building trust in machine learning systems, aimed at providing insights into the working of complex neural networks that are otherwise opaque to a user. There are a plethora of existing solutions addressing various aspects of interpretability ranging from identifying prototypical samples in a dataset to explaining image predictions or explaining mis-classifications. While all of these diverse techniques address seemingly different aspects of interpretability, we hypothesize that a large family of interepretability tasks are variants of the same central problem which is identifying \emph{relative} change in a model's prediction. This paper introduces MARGIN, a simple yet general approach to address a large set of interpretability tasks MARGIN exploits ideas rooted in graph signal analysis to determine influential nodes in a graph, which are defined as those nodes that maximally describe a function defined on the graph. By carefully defining task-specific graphs and functions, we demonstrate that MARGIN outperforms existing approaches in a number of disparate interpretability challenges.

==> background.tex <==
%i.e., $f:\mathcal{N}\mapsto \mathbb{R}^N$

In our experiments, we will restrict our analysis to undirected graphs with real-valued functions, but both the theory and inference algorithms generalize to directed graphs and complex-valued functions as well \cite{sandryhaila2013discrete}. In practice, it is convenient to represent these functions as a vector (or a row major matrix for high dimensional functions) indexed by the nodes, assuming a fixed ordering that is consistent across all the graph operators.

Formally, an undirected weighted graph is represented by the triplet $\mathcal{G} = (\mathcal{V}, \mathcal{E}, \mathbf{W})$, where $\mathcal{V}$ denotes the set of nodes, $\mathcal{E}$ denotes the set of edges and $\mathbf{W}$ is the adjacency matrix that specifies the weights on the edges, where $\textbf{W}_{n,m}$ corresponds to the weight on the edge between nodes $v_n$ and $v_m$. Let $\mathcal{N}_{n} = \{m | \mathbf{W}_{n,m} \neq 0\} $ define the neighborhood of node $v_n$, i.e. the set of nodes connected to it. The fundamental component of graph analysis is the normalized graph Laplacian $\mathbf{L}$, which is defined as $\mathbf{I} - \mathbf{D}^{-1/2}\mathbf{W} \mathbf{D}^{-1/2}$, where $\mathbf{D}_{nn} = \sum_m \mathbf{W}_{n,m}$ is the degree matrix and $\mathbf{I}$ denotes the identity matrix.

\paragraph{Graph Signal Processing:} We use the notation and terminology from \cite{sandryhaila2013discrete} in defining an operator analogous to the \emph{time-shift} or \emph{delay} operator in classical signal processing. During a graph shift operation, the function $\mathbf{f}(n)$ at node $v_n$ is replaced by a weighted linear combination of its neighbors: $\hat{\mathbf{f}} = \mathbf{A}\mathbf{f}$, where $\mathbf{A}$ is the graph shift operator, which is the simplest, non-trivial graph filter. Commonly used choices for $\mathbf{A}$ include the adjacency matrix $\mathbf{W}$, transition matrix $\mathbf{D}^{-1}\mathbf{W}$ and the graph Laplacian $\mathbf{L}$.

The set of eigenvectors of the graph shift operator is referred to as the graph Fourier basis, $\mathbf{A} = \mathbf{U} \mathbf{\Lambda} \mathbf{U}^T$, where $\mathbf{U} \in \mathbb{R}^{N\times N}$, and the Fourier transform of a signal $\mathbf{x} \in \mathbb{R}^N$ is defined as $\mathbf{U}^T \mathbf{x}$. The ordered eigenvalues corresponding to these eigenvectors represent frequencies of the signal, with $\lambda_1$ to $\lambda_N$ representing the smallest to largest frequencies. The notion of frequency on the graph corresponds to the rate of change of the function across nodes in a neighborhood. A higher change corresponds to a high frequency, while a smooth variation corresponds to a low frequency. In this context, the graph filtering using a graph shift operator corresponds to a \emph{low pass} filter that dispenses high frequency components in the function. Similarly, a \emph{high pass} filter can also be easily designed by removing the low frequency components from the original signal as $\mathbf{f}_{high} = \mathbf{f} - \hat{\mathbf{f}}$.



==> corrupt_sup.tex <==
\begin{figure}[!htb]
  \includegraphics[width=0.9\linewidth,clip=False,trim=-10 20 50 30]{figs/Kaggle_flipped_labels.png}
  \caption{Using MARGIN to detect incorrectly labeled samples from Kaggle Dogs vs Cats dataset \protect\cite{elson2007asirra}}
  \label{fig:kaggle}
\end{figure}

We show additional experiments for the task of identifying corrupted labels,  on a subset of the Kaggle Dogs v Cats dataset \cite{elson2007asirra} \footnote{\url{https://www.kaggle.com/c/dogs-vs-cats}}, with 3,000 images of almost equally sized classes. While the previous experiment showed improvement over state-of-the-art, we show that when classes are somewhat more balanced, the performance gain using MARGIN is significantly higher. From Figure \ref{fig:kaggle}, we observe that the graph-based sampling clearly outperforms the baselines by providing a recall of nearly 1.0 after observing only $\approx$ 20\% of the samples. In comparison, with the same number of samples, the state-of-the-art Influence Functions method has a recall of around $0.84$.


==> saliency_algo.tex <==
In this section, we show additional examples of explanations generated using MARGIN, based on predictions from AlexNet. As shown in Figure \ref{fig:saliency_maps_add}, MARGIN produces consistently interpretable explanations across different classes, while being sparse and not heavily dependent on features whose correlations to the class label are not obvious. Broadly, the explanations corroborate strongly with state-of-the-art techniques including Grad-CAM. 
\begin{figure*}[!htb]
	\centering
	\includegraphics[width=.8\linewidth,clip=True,trim=0 0 0 0]{figs/saliency.pdf}
	\vspace{-10pt}
	\caption{Our approach identifies the most salient regions in different classes for image classification using AlexNet. From top to bottom: original image, MARGIN's explanation overlaid on the image, and Grad-CAM's explanation. Note our approach yields highly specific, and sparse explanations from different regions in the image for a given class.}
	\label{fig:saliency_maps_add}
	\vspace{-10pt}
\end{figure*}

